Entangling Quantum Memories via Heralded Photonic Bell Measurement

A common way to entangle quantum memories is via photonic entanglement swaps. Each of two memories, connected by an optical channel, emits a photonic qubit entangled with itself, and the photonic qubits undergo an entanglement swap on a beamsplitter in the middle of the channel. We compare two choices of encoding of the photonic qubit: single rail and dual rail. At low channel loss the dual-rail scheme outperforms the single rail scheme. However, as expected, the high-loss rate asymptote for the dual rail scheme scales quadratically worse with loss compared with single rail. Considering the following non-idealities: imperfect mode matching at the swap, carrier-phase mismatch across the interfered photonic qubits, and detector excess noise, we evaluate the density operator of the heralded two-qubit entangled state. We calculate a lower bound on its distillable entanglement per copy, and its Fidelity (with the ideal Bell state). For both schemes, imperfect swap-visibility results in a constant-factor decrease in the rate, while excess noise results in a dropoff of distillable entanglement beyond a certain total channel loss threshold, to zero. Despite the single-rail scheme's better rate-loss scaling, it is more severely affected by excess noise. The single-rail scheme is adversely affected by stochastic carrier-phase mismatch, which does not affect the dual-rail scheme. We study entanglement distillation on the heralded noisy entangled states for both methods, and outline a suite of quantum networking studies that our work could incite.

==> commented.tex <==
\section{Complete State Description}
\subsection{Dual rail swapped state}
Assume the initial spin-photon entangled qubit state to be
\begin{align}
	\ket{\psi}=\sqrt{\gamma}\ketup\ket{0}+\sqrt{1-\gamma}\ketdown\ket{1})
\end{align}
henceforth we shall refer to $ \gamma $ as the qubit initialization parameter. 

This note focusses on the performance of the entanglement swapping between two copies of $ \ket{\psi} $. The entanglement swapping step is carried out between one qubit of each ebit, after they have been transmitted to a common physical location. 
For the most general case, we work with different qubit initialization parameters $ (\gamma_A,\gamma_B) $ for each ebit initialized by two parties (say Alice and Bob), along with generalized transmission loss parameter $ \eta_A $ and $ \eta_B $ on either side respectively. We also incorporate the effect of a random phase imparted on an optical mode through the generating unitary $ U_\theta=\exp(\i\phi) $ where  $ \phi\sim\mathcal{N}(0,\epsilon), \epsilon\ll1 $. Such an operator would act on both the transmitted photonic qubits, however since the qubits are equivalent upto a global phase factor, we may abstract it to being a single random phase on (say) Alice's qubit. For example, the action of the random phase operator on Alice's state before loss is $  (\sqrt{\gamma}\ketup\ket{0}+e^{i\theta} \sqrt{1-\gamma}\ketdown\ket{1})$. 
%The parameter $ \theta $ is a random variable drawn from a random distributiion of small variance (say $ \theta\sim\mathcal{N}(0,\epsilon) $). 


A successful entanglement swap is heralded by the detection of a $ [1,0] $ or $ [0,1] $ click pattern on the heralding detectors. Let us assume, that the detectors have a detection efficiency of $ \eta_d $ and suffers from an net excess noise of $ P_d $  photons per qubit slot. The heralded spin-spin entangled state is then given as, 
\begin{align}
	\hat{\sigma}=g_1\cdot\outprod{\uparrow,\uparrow}+\highlightC{g_2\cdot\outprod{\uparrow,\downarrow} +g_3\outprod{\downarrow,\uparrow}+g_4\proj{\uparrow,\downarrow}{\downarrow,\uparrow} + g_4^* \proj{\downarrow,\uparrow}{\uparrow,\downarrow}} + g_5 \cdot\outprod{\downarrow,\downarrow},
\end{align}
where the \highlightC{cyan} terms represent the desired spin-spin entangled state. The coefficients $ g_k $ are given in terms of the parameters as,
\begin{subequations}
	\begin{align}
		g_1&=P_d (1-P_d)\gamma_A\gamma_B\\
		g_2&=\frac{1}{2}(1 - P_d)^2 \,\gamma_A \,(1 - \gamma_B) \,\eta_B \eta_d + (1 - 
		P_d) P_d\, \gamma_A (1 - \gamma_B) (1 - \eta_B \eta_d)\\
		g_3&=\frac{1}{2} (1 - P_d)^2\, (1 - \gamma_A) \, \gamma_B \, \eta_A \eta_d + (1 - 
		P_d) P_d\,  (1 - \gamma_A) \gamma_B (1 - \eta_A \eta_d)\\
		g_4&=\frac{1}{2} \, \eta_d e^{i\theta}(1 - P_d)^2 \sqrt{\gamma_A(1 - \gamma_A)} \sqrt{\gamma_B(
			1 - \gamma_B)}  \sqrt{\eta_A \eta_B }; \quad \theta\sim\mathcal{N}(0,\epsilon)\\
		g_5&=(1 - P_d) P_d (1 - \gamma_A) (1 - \gamma_B) (1 - \eta_A \eta_d) (1 \
		- \eta_B \eta_d) \nonumber \\
		&\quad+ \frac{1}{2} \eta_d (1 - P_d)^2 (1-\gamma_A)(1-\gamma_B)\left(\eta_A+\eta_B-2\eta_A\eta_B\eta_d\right)
	\end{align}
\end{subequations}

The fidelity of the state $ \hat{\tilde{\sigma}} $ w.r.t. the ideal spin-spin Bell pair $ (\ket{\uparrow,\downarrow}+\ket{\downarrow,\uparrow})/\sqrt{2} \equiv\ket{\Psi^+}$ when $ P_d=0; \, \eta_d=1 $ is given as, 
\begin{align}
	F(\hat{{\sigma}},\ket{\Psi^+})=	\frac{\eta_A\gamma_B(\gamma_A-1)+\eta_B\gamma_A(\gamma_B-1)-2 \sqrt{\gamma_A(1-\gamma_A)} \sqrt{\gamma_B(1-\gamma_B)} \sqrt{\eta_A\,\eta_B} \cos \theta
	}
	{2 (\gamma_B-1) \eta_B+2 (\gamma_A-1) \eta_A+4 (\gamma_A-1) 
		(\gamma_B-1) \eta_B\eta_A  }
\end{align}

For certain specific cases, we report the following analytic formulae,
\begin{enumerate}
	\item $  \eta_A=\eta_B=1$ \begin{align}
		F(\hat{{\sigma}},\ket{\Psi^+}) =\frac{1}{2}+\frac{\sqrt{\gamma_A(1-\gamma_A)} \sqrt{\gamma_B(1-\gamma_B)} \cos \theta}{\gamma_A+\gamma_B-2\gamma_A\gamma_B} 
	\end{align} 
	\item $ \gamma_A=\gamma_B ; \eta_A=\eta_B=1$
	\begin{align}
		F(\hat{{\sigma}},\ket{\Psi^+}) =(1+\cos\theta)/2
	\end{align}
\end{enumerate}

\section{Evaluating the Ultimate Rate: Reverse Coherent Information}
\subsection{Noiseless Entanglement Swap: $ P_d=0 $}

We try to uncover an analytical understanding to the ultimate rate. Specifically considering $ P_d=0$ and setting $ \gamma_A=\gamma_B=\gamma; \eta_A=\eta_B=\sqrt{\eta}  $, the final state can be expressed as,
\begin{align}
	\tilde{\sigma}=\mathbf{N_0}^{-1} \left(g'_1\cdot\outprod{\uparrow,\downarrow} +g'_1\outprod{\downarrow,\uparrow}+g'_2\proj{\uparrow,\downarrow}{\downarrow,\uparrow} + g^{'*}_2 \proj{\downarrow,\uparrow}{\uparrow,\downarrow} + g'_3 \cdot\outprod{\downarrow,\downarrow}\right),
	\label{eqn:finalst}
\end{align}
where $ \mathbf{N_0}=(\sqrt{\eta}\,(1-\gamma)(1-(1-\gamma)\sqrt{\eta})) $ and the coefficients are,
\begin{subequations}
	\begin{align}
		g'_1&= \frac{1}{2} \,\gamma \,(1 - \gamma) \,\sqrt{\eta} ; \quad 
		g'_2=\frac{1}{2} \,  e^{i\theta} \gamma(1 - \gamma)  \sqrt{\eta}; \quad \theta\sim\mathcal{N}(0,\epsilon);\quad
		g'_3=  (1-\gamma)^2\left(\sqrt{\eta}-\eta \right).
	\end{align}
\end{subequations}


The fidelity and the probability of generation of $ \tilde{\sigma} $ in Eq.~\eqref{eqn:finalst}, in terms of these parameters is given as 
\begin{subequations}
	\begin{align}
		&\text{Fidelity:}\qquad F(\tilde{\sigma},\ket{\Psi^+})= \frac{2g'_1+g'_2+g^{'*}_2}{\mathbf{N_0}}\\
		&\text{Prob. of Generation:}\qquad P_{gen}(\tilde{\sigma})=\mathbf{N_0}=(\sqrt{\eta}\,(1-\gamma)(1-(1-\gamma)\sqrt{\eta}))
	\end{align}
\end{subequations}

To understand the ultimate rate of entanglement swap for the present formulation, we shall use the reverse coherent information (RCI) quantity of a quantum state. This gives a \textit{lower} bound to the distillable entanglement of a quantum state, and is defined for a bi-partite quantum state $ \rho_{AB} $ as $ I_R(\rho_{AB}) =S(\Tr_A(\rho_{AB})))-S(\rho_{AB})$. Hence, the reverse coherent information for the final state in Eq.~\eqref{eqn:finalst} is given as,
\begin{align}
	I_R(\tilde{\sigma})=h_2(s/2)-h_2(s),
	\label{eqn:rci_finalst}
\end{align} where $ h_2(x) \equiv=-x\ln x-(1-x)\ln(1-x);\,x\in[0,1]$ is the binary entropy function and the variable $ s $ stands for,
\begin{align}
	s=\frac{\gamma}{1-(1-\gamma)\sqrt{\eta}}.
\end{align}

Note that the RCI calculated in Eq.~\ref{eqn:rci_finalst} is the ultimate rate iff the state in Eq.~\ref{eqn:finalst} is \textit{successfully} heralded. Additionally to obtain the ultimate rate in terms of distilled ebit per second, we have to account for the bandwidth ($ W $)of the source. Hence the desrired ultimate rate is evaluated by the product, \begin{align}
	I_R(\tilde{\sigma})\times P_{gen}(\tilde{\sigma}) \times W \equiv\mathcal{R}(\eta,\gamma).
	\label{eqn:ult_rate}
\end{align}

Note that unlike $ \eta $ in Eq.~\ref{eqn:ult_rate}, which is a protocol parameter, $ \gamma $ can be optimized to maximize the rate. Fig.~\ref{fig:ultrate} shows the plot of $ \mathcal{R}(\eta,\gamma) $ w.r.t. $ \eta $ when $ \gamma $ is (numerically) optimized for each value of $ \eta $. Comparison of the ultimate rate of entanglement swap for the single-rail encoded qubit (purple) with the dual-rail qubit (blue) and the ultimate rate for the channel given by $ -W\times \log(1-\sqrt{\eta})  $.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.6\linewidth]{ultrate_v1}
	\caption{ Comparison of the ultimate rate of entanglement swap for the single-rail encoded qubit (purple) with the dual-rail qubit (blue) and the ultimate rate for the channel given by $ -W\times log(1-\sqrt{\eta})  $.}
	\label{fig:ultrate}
\end{figure}

\section{Numerical Maximization}
To understand the observed trend, we plot the value of the optimal $ \gamma $ vs. $ \eta $ in Fig. ~\ref{fig:gammaveta}. Additionally, In Fig.  we  plot  $ \mathcal{R}(\eta,\gamma) $ w.r.t. $ \eta $, with its underlying components $ I_R(\cdot) $ and $ P_{gen}(\cdot)$. For this analysis we arbitrarily set $ W=1 $, as it is simply an overall multiplier.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.6\linewidth]{optimalgamma_v1}
	\caption{ Plot of the optimal $ \gamma $ that maximizes $ \mathcal{R}(\cdot) $ vs. $ \eta $.}
	\label{fig:gammaveta}
\end{figure}

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.6\linewidth]{ultdec_v1}
	\caption{ Plot of $ \mathcal{R}(\eta,\gamma) $ w.r.t. $ \eta $, with its underlying components $ I_R(\cdot) $ and $ P_{gen}(\cdot)$. For this analysis we arbitrarily set $ W=1$. }
	\label{fig:compveta}
\end{figure}

Based on Fig.~\ref{fig:compveta}, there are two scaling regimes for $ \mathcal{R}(\cdot) $.

For $ \eta $ close to 1, the $ P_{gen} $ is approximately given  by $ \gamma(1-\gamma) $, which is maximized for $ \gamma=1 $. Additionally, $ I_R(\cdot) $ is close to its maximum value of $ \ln2 $, which is that of a perfect ebit. As $ \eta $ decreases, the $ P_{gen} $ is maximized for an increasing value of $ \gamma $, as it is mostly dominated by the $ (1-\gamma) $ factor. For $ I_R(\cdot) $, the underlying function $ h_2(s/2) -h_2(s)$ is increasing as $ \gamma\rightarrow1 $. We note that other than $ \eta=1 (0 \text{ dB})$, $ s $ is strictly sub-unity. Hence, increasing $ \gamma  $ raises $ s $, by increasing the numerator and giving  increased weight to the $ (1-\gamma)\sqrt{\eta}$ term as well. 

In the regime of high loss ($ \eta\approx 0 $), $ I_R(\cdot) $ is approximately given by  $ h_2(\gamma/2)-h_2(\gamma) $. Hence $ \gamma $ closer to 1 is the optimal value. $ P_{gen}$ sets the scaling (notably $ \propto \sqrt{\eta} $).




\subsubsection{Analytic Maximization}
Our objective is to maximize $ \mathcal{R}(\eta,\gamma) $ w.r.t. $ \gamma $. The evaluation of $ d\mathcal{R}(\cdot)/d\gamma $ gives us the relations,
\begin{subequations}
	\begin{align}
		I_R(\tilde{\sigma})\,\frac{d}{d\gamma} P_{gen}(\tilde{\sigma})&= \left[h_2(s/2)-h_2(s)\right]\times \left(2(1-\gamma)\eta-\sqrt{\eta}\right) \equiv F_1 \label{eqn:simp1_eq1}\\
		P_{gen}(\tilde{\sigma}) \,\frac{d}{d\gamma} I_R(\tilde{\sigma})&= \mathbf{N_0}\times \left(\frac{1}{2}\ln \frac{1-s/2}{s/2}-\ln \frac{1-s}{s}\right)\times \frac{1-\sqrt{\eta}}{(1-(1-\gamma)\sqrt{\eta})^2}\equiv F_2\label{eqn:simp1_eq2}
	\end{align}
\end{subequations}
Now let us assume, $ \eta=1-\varepsilon\Rightarrow\sqrt{\eta}=\sqrt{1-\varepsilon} =1-\epsilon/2+\mathcal{O}(\varepsilon^2)$. This lets us simplify $ s $ as 
\begin{align}
	\begin{split}
		s=\frac{\gamma}{1-(1-\gamma)\sqrt{\eta}}&=\gamma\times\left(1-\sqrt{\eta}+\gamma\sqrt{\eta}\right)^{-1}\\
		&\approx \gamma\times\left(1-(1-\ve/3)+\gamma(1-\ve/2)\right)^{-1}  \\
		&\approx \gamma\times\left[\gamma(1-\ve/2+\ve/(2\gamma))\right]^{-1}\\
		&\approx1+\ve/2-\ve/(2\gamma) = 1-\delta \;(\text{say})
	\end{split}
\end{align}

We may now use the approximation, $ h_2(s)\approx h_2(1-\delta) =-\delta\ln \delta+\delta-{\delta^2}/{2}-{\delta^3}/{6}+\mathcal{O}(\delta^4)$ and $ h_2(s/2)\approx h_2(1/2-\delta/2)=\ln 2-\delta^2/2 +\mathcal{O}(\delta^4)$ to simplify Eq.~\eqref{eqn:simp1_eq1} as
\begin{align}
	\begin{split}
		F_1&\approx (\ln2-\delta^2/2+\delta\ln\delta-\delta+\delta^2/2+\delta^3/6)\times \left( 2(1-\gamma)(1-\ve)-(1-\ve/2)\right)\\
		&=(\ln2+\delta\ln\delta-\delta+\delta^3/6)\times \left( 2(1-\gamma)(1-\ve)-(1-\ve/2)\right)
	\end{split}
	1\end{align}

\begin{align}
	\begin{split}
		F_2&=\frac{(1-\gamma)\sqrt{\eta}\,(1-\sqrt{\eta})}{(1-(1-\gamma)\sqrt{\eta})}\left(\frac{1}{2}\ln \frac{2-s}{s}-\ln \frac{1-s}{s}\right)\\
		&\approx \frac{(1-\gamma)(1-\ve/2)\,(\ve/2)}{(1-(1-\gamma)(1-\ve/2))}\times \left(\frac{1}{2}\ln \frac{1+\delta}{1-\delta}-\ln \frac{\delta}{1-\delta}\right)\\
		&\approx  \frac{(1-\gamma)(1-\ve/2)\,(\ve/2)}{(1-(1-\gamma)(1-\ve/2))}\times \left(-\ln \delta -\delta^2/2 +\mathcal{O}(\delta^4)\right)\\
		&\approx  \frac{(1-\gamma)(1-\ve/2)\,(\ve/2)}{\gamma}\times \left(1+\ve/2-\ve/2\gamma\right)\times \left(-\ln \delta -\delta^2/2 +\mathcal{O}(\delta^4)\right)
	\end{split}
\end{align}

Putting it together for an extrema, we have to solve for $ F_1+F_2=0 $, which is a transcendental equation.

%%% Added  Feb 6
\begin{itemize}
	\item The single rail swap outperforms the dual rail encoded swap (with a scaling of $ \mathcal{O}(\eta) $) in the high loss limit $ (\eta\ll1) $. However, in the low loss limit ($ \sqrt{\eta}<8 $dB), the dual rail swap outperforms the single rail swap.
	
	\item For $ P_d>0 $, $ \mathcal{R}(\rho_{AB}) $ crashes to zero at a finite value of $ \eta $, indicating a maximum range for entanglement swapping in the presence of excess noise. The single rail swapped state is more susceptible to excess noise, i.e., for same $P_d$, $ \mathcal{R}(\rho_{AB}) $ crashes to zero for lower loss for the single rail swapped state.

    \item Phase mismatch reduces the fidelity of the single rail swapped state as $ F\rightarrow F\times(1+\cos(\arg\mathcal V))/2 $, but does not affect the dual rail swapped state.
	
	\item Swapping with $ |\mathcal{V}|<1$, does not affect $ P_{\mathrm{succ.}} $ but affects the  state quality  $ I(\rho_{AB}) $, which is lower than the ideal unity visibility state for all  $ \eta$.
\end{itemize}
